Low Light Video Enhancement by Learning on Static Videos with Cross-Frame Attention

The design of deep learning methods for low light video enhancement remains a challenging problem owing to the difficulty in capturing low light and ground truth video pairs. This is particularly hard in the context of dynamic scenes or moving cameras where a long exposure ground truth cannot be captured. We approach this problem by training a model on static videos such that the model can generalize to dynamic videos. Existing methods adopting this approach operate frame by frame and do not exploit the relationships among neighbouring frames. We overcome this limitation through a selfcross dilated attention module that can effectively learn to use information from neighbouring frames even when dynamics between the frames are different during training and test times. We validate our approach through experiments on multiple datasets and show that our method outperforms other state-of-the-art video enhancement algorithms when trained only on static videos.

==> Images/supplymentary.tex <==
\label{chap:Supplementary}
\section{Architecture of Fusion Module}

\label{sec:Fusion}
\begin{figure}[h]
% \vspace{-1cm}
\centering
\bmvaHangBox{{\includegraphics[width=12.4cm]{Images/fusion_blkdgm.png}}}
% \includegraphics[scale=0.4]{Base_model_block.png}
\caption{Block diagram illustrating our fusion module}
\label{fig:fusion}
\end{figure}
In this section, we describe the adaptive fusion for $N$ attention maps (see Figure \ref{fig:fusion}), $\{A^1, A^2, \ldots, A^N\}$.
We pass each of these maps through a convolutional layer and get $W^n$ for $n=1,2,\ldots,N$, where each $W^n$ is a single channel map. The same map will be used to determine the weights for all the channels in the attention map. Finally, to obtain the mixing weights for $A^n$ at each location, we apply a softmax operation at each spatial location across all the $N$ maps. The resulting weights are used to fuse the attention map followed by the residual channel attention block (RCAB). 

% \begin{equation}
% W\textsubscript{2} = SoftMax(cat((A\textsuperscript{1}\textsubscript{1},A\textsuperscript{2}\textsubscript{1})))
% \end{equation}

% Now we channel wise split W\textsubscript{2} to get W\textsuperscript{1}\textsubscript{1} and W\textsuperscript{2}\textsubscript{1} 

% \begin{equation}
% W\textsuperscript{1}\textsubscript{C} = Repeat(W\textsuperscript{1}), W\textsuperscript{2}\textsubscript{C} = Repeat(W\textsuperscript{2})
% \end{equation}
% At last to get fused map, we take weighted sum of given maps with weighted maps.
% \begin{equation}
% A\textsuperscript{Fused} = A\textsuperscript{1} \cdot W\textsuperscript{1}\textsubscript{C} +  A\textsuperscript{2} \cdot W\textsuperscript{2}\textsubscript{C}
% \end{equation}


% Attention Map A she ows the correlation between elements in the feature map of reference frame and other feature map of temporal frame. LN represents layer norm Output of this module can we formulated as:
% \begin{equation}\label{eq4}
% X\textsuperscript{out} =  LN(LinearLayer(LN(CrossAttention(Q\textsuperscript{1},K\textsuperscript{2}, V\textsuperscript{2})) + X\textsuperscript{1}))
% \end{equation}


\section{Ablation on DRV-SM Dataset}\label{sec:Ablation}
We evaluated the importance of various components of our model, in particular, cross-attention and dilated cross-attention with respect to our base line model on the DAVIS dataset in the main paper. Here we present similar results on the DRV-SM dataset using the ST-RRED quality measure in Figure \ref{BaseAttnModule}. We see consistent improvements with respect to our ideas even in the DRV-SM dataset.  

\begin{figure}[h]
\label{BaseAttnModule}
% \vspace{-1cm}
\centering
\bmvaHangBox{{\includegraphics[width=6.2cm]{Images/Ablation_All.jpg}}}
% \includegraphics[scale=0.4]{Base_model_block.png}
\caption{Ablation Evaluation on our model with DRV-SM dataset}
\end{figure}

%\section{Performance on Static DRV Dataset}
%Although our primary objective was in the performance evaluation of the dynamic videos, here we also evaluate the performance of our method on the static videos in the DRV dataset referred to as Static DRV dataset \cite{SMID}. The models are all trained on the same static sequences mentioned in Setting 1 in the main paper, but now evaluated on 49 static video sequences. In particular, we test on the first 10 frames from each of these static sequences in Table \ref{DDRV Results}. We evaluate using SSIM and PSNR since there is no motion in the video sequences. We note that there is no clear winner with respect to different performance measures and our approach is competitive with the best. To summarize, our model achieves a stable performance across both static and dynamic test videos. 

% \begin{table}[h]
% \label{DDRV Results}% is used to refer this table in the text
% \caption{Performance On Static DRV Dataset} % title of Table
% \centering % used for centering table
% \begin{tabular}{c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines

% Methods  & SSIM \uparrow & PSNR \uparrow\\ [1ex] % inserts table
% \hline % inserts single horizontal line
% SMID\cite{SMID}   & \textbf{0.63}  & 28.43\\
% MBLLVEN\cite{MBLLEN}   & 0.58  & 28.36\\
% FastDVDNet\cite{FastDVDnet}  & 0.62 & 28.52\\
% VRT\cite{VRT}  & 0.53 & 28.37\\
% %Our Base Model & \textbf{0.63} & \textbf{28.55} \\
% %Our Without Dilation  & 0.62 & 28.50\\
% Ours  & 0.61 & \textbf{28.53}\\[1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \label{DDRV Results}% is used to refer this table in the text
% \caption{Performance On Static DRV Dataset} % title of Table
% \centering % used for centering table
% \begin{tabular}{c c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines

% Methods  & SSIM \uparrow & ST-RRED \downarrow & PSNR \uparrow\\ [1ex] % inserts table
% \hline % inserts single horizontal line
% SMID\cite{SMID}   & \textbf{0.63} & 859 & 28.43\\
% MBLLVEN\cite{MBLLEN}   & 0.58 & 537 & 28.36\\
% FastDVDNet\cite{FastDVDnet}  & 0.62 & \textbf{457} & 28.52\\
% VRT\cite{VRT}  & 0.53 & 786 & 28.37\\
% Our Base Model & \textbf{0.63} & 736 & \textbf{28.55} \\
% Our Without Dilation  & 0.62 & 698 & 28.50\\
% Ours  & 0.61 & 794 & 28.53\\[1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \end{table}

\section{Comparison with Data Generation based Methods}
We now describe our experiments in comparing with a data generation method for training low light video enhancement \cite{CycleGAN}. SIDGAN adopts a two-step procedure to generate realistic low light videos from high quality videos in the Vimeo dataset \cite{vimeo}. In particular, a pair of cycle-GANs is used where the first cycle-GAN generates sensor specific long exposure video frames from which a second cycle-GAN generates short exposure video frames. Thus, paired labelled data is created which can be used to train deep network. However, we observe that each cycle-GAN generates very poor quality images in our experiments as shown in Figure \ref{fig:sidgan}. Thus we did not proceed with training the enhancement model. We believe that poor quality of video frames could perhaps be attributed to the larger image resolutions that we operate with when compared to SIDGAN \cite{CycleGAN}. Due to memory constraints, we are not able to experiment with larger patch sizes in their model which could potentially improve performance. 

\begin{figure*}[h]
\begin{center}
  \begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/gt_in.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/gt_out.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/ll_in.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/ll_out.jpg}}
\end{minipage}
\\
  \begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/gt_in_1.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/gt_out_1.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/ll_in_1.jpg}}
\end{minipage}
\hfill
\begin{minipage}[b]{0.245\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{Images/ll_out_1.jpg}}
\end{minipage}

\caption{Examples of images generated using the SIDGAN \cite{CycleGAN}. First column are the ground truth images from the Vimeo dataset. Second column contains outputs from first stage of SIDGAN of transforming Vimeo ground truth to sensor specific ground truths from the DRV dataset. Third column contains ground truth images from the DRV dataset and the last column contains outputs of the second stage of the SIDGAN of transforming images from third column to low light from the DRV dataset. Note that the generated images appear unnatural.}
\label{fig:analysis}
\end{center}
\label{fig:sidgan}
\end{figure*}
